The Intended Uses of Automated Fact-Checking Artefacts: Why, How and Who

Automated fact-checking is often presented as an epistemic tool that fact-checkers, social media consumers, and other stakeholders can use to fight misinformation. Nevertheless, few papers thoroughly discuss how. We document this by analysing 100 highly-cited papers, and annotating epistemic elements related to intended use, i.e., means, ends, and stakeholders. We find that narratives leaving out some of these aspects are common, that many papers propose inconsistent means and ends, and that the feasibility of suggested strategies rarely has empirical backing. We argue that this vagueness actively hinders the technology from reaching its goals, as it encourages overclaiming, limits criticism, and prevents stakeholder feedback. Accordingly, we provide several recommendations for thinking and writing about the use of fact-checking artefacts.

==> data/data_actors_by_year.tex <==
year	algorithm	citizen_journalists	engineers_and_curators	law_enforcement	media_consumers	none	professional_journalists	scientists	technical_writers
2008	0	0	0	100.0	0	0	0	0	0
2009	0	0	0	0	0	100.0	0	0	0
2014	0	100.0	0	0	100.0	100.0	100.0	0	0
2015	0	25.0	0	0	0	50.0	50.0	25.0	0
2016	20.0	0	0	0	20.0	100.0	20.0	20.0	0
2017	0	0	0	0	0	100.0	27.272727272727273	0	0
2018	8.695652173913043	0	0	0	17.391304347826086	91.30434782608695	26.08695652173913	4.3478260869565215	0
2019	0	6.666666666666667	13.333333333333334	0	6.666666666666667	86.66666666666667	26.666666666666668	0	0
2020	0	0	0	0	3.5714285714285716	89.28571428571429	14.285714285714286	7.142857142857143	3.5714285714285716
2021	0	0	0	0	9.090909090909092	90.9090909090909	45.45454545454545	9.090909090909092	0
